Variable Length Embeddings

In this work, we introduce a novel deep learning architecture, Variable Length Embeddings (VLEs), an autoregressive model that can produce a latent representation composed of an arbitrary number of tokens. As a proof of concept, we demonstrate the capabilities of VLEs on tasks that involve reconstruction and image decomposition. We evaluate our experiments on a mix of the iNaturalist and ImageNet datasets and find that VLEs achieve comparable reconstruction results to a state of the art VAE, using less than a tenth of the parameters.

==> related.tex <==
\section{Related Works}

\paragraph{Autoencoders} Autoencoders play a central role in the VLE framework. A central feature of autoencoders is that they can be trained in an unspervised fashion. This unsupervised training can be a powerful way to learn features from a data distribution without the burden of labeling these features by hand. For instance, a number of works \citep{Thewlis_2017_ICCV,jakab2018unsupervised,Zhang_2018_CVPR,Lorenz_2019_CVPR} have deployed autoencoders to learn object landmarks in an unsupervised fashion. Another popular task to which autoencoders have been applied is generative modeling. \citet{kingma2013auto} introduced variational autoencoders as a means to learn a latent distribution of the training data. This latent distribution can then used to sample images from the data distribution. Since then, autoencoders have been a popular substrate for many generative modeling tasks \citep[e.g.,][]{vahdat2020nvae,luhman2023high}.

\paragraph{Recurrent Models}

\paragraph{Diffusion Models} Finally, given the popularity of diffusion models, it is hard not to the parallels of our work to that of diffusion models. Each successive latent space encoding adds increasing detail to the image similar to the way each additional diffusion step does. We feel that diffusion models has it shortcomings in its inability to separate the understanding of objects and believe this often leads to poorly generated images when prompted for a subject that is less seen in the training set.
